DAL: Dynamic Angular Loss for Imbalanced Medical Image Classification

Class imbalance remains a major obstacle in medical image classification, where rare but clinically important classes are often overshadowed by majority categories. Although current strategies for reducing bias, including angle-based softmax (ABS) losses, offer strong discriminative features, their behavior in settings with a small number of severely imbalanced classes remains insufficiently understood. Previous approaches that estimate the intrinsic parameters of ABS rely on the assumption of many classes, which does not hold in medical settings. We derive data-driven upper and lower bounds for the scale parameter and an upper bound for the angular margin using negative-angle statistics, and use these to drive a batch-adaptive angular margin (BAAM), which we combine with dynamically-weighted cross entropy (DWCE) to define our dynamic angular loss (DAL). Across four highly imbalanced medical image classification benchmarks spanning dermatology, ophthalmology, and gastrointestinal endoscopy, our method consistently achieves superior balanced accuracy and the lowest coefficient of variation of per-class recall. Although this entails a small performance reduction on majority classes, the gains on minority categories are substantial, yielding a reliable and equitable overall classifier. Our source code is available at: https://github.com/msalman95/DAL.

==> sections/preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\usepackage{url}
\usepackage{color}
\usepackage[dvipsnames,svgnames]{xcolor}
\usepackage{graphicx}
\usepackage{float}
\usepackage{xspace}
\usepackage{lipsum}
\usepackage{amsmath,amssymb}
%\usepackage{titlesec}
\usepackage{gensymb}
\usepackage[hidelinks]{hyperref}

\usepackage[listofformat=parens, justification=centering, subrefformat=subparens]{subfig}  % have multiple floats in one figure


\usepackage{framed,multirow}
\usepackage[point]{fltpoint}
\usepackage{textcomp}
\usepackage{ifthen}
\usepackage{latexsym}
\usepackage{enumerate}

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%\newcommand{\TODO}[1]{}

\newcommand{\figref}[1]{Fig.~\ref{#1}\xspace}
%\renewcommand{\subfigref}[1]{Fig.~\subref{#1}\xspace}
\newcommand{\tabref}[1]{Tab.~\ref{#1}\xspace}
%\renewcommand{\subtabref}[1]{Tab.~\subref{#1}\xspace}
\newcommand{\secref}[1]{Sec.~\ref{#1}\xspace}
\newcommand{\appxref}[1]{Appx.~\ref{#1}}

%%
%% disable for camera ready / submission by uncommenting these lines
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}
\usepackage{amsmath}
\newcommand{\T}{\mathsf{T}} % or \mathrm{T}


\newcommand\Caption[3][]{\caption[#2]{\label{#1}\textsc{#2}.\small#3}}
%\newcommand{\rednum}[1]{{\color{red}#1}}
\newcommand{\rednum}[1]{\textbf{#1}}

\newcommand{\ie}{\textit{i.\,e.}\xspace}
\newcommand{\eg}{\textit{e.\,g.}\xspace}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
\usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}


==> tables/combination.tex <==
\begin{table}[t]
\floatconts{tab:angular-only-results}
{\color{blue}\Caption{Angular Loss with Different Loss Functions}{
    Test set performance when combining the angular formulation in \eqref{eq:adacos} with $S=4$ with different loss functions from the literature.
    Results are reported as the mean over five runs.\vspace*{-4ex}
}}
{
\scriptsize
\begin{tabular}{lccccccc}
\bfseries Method 
& \bfseries Acc 
& \bfseries F1 
& \bfseries BAcc 
& \bfseries IBA$_{0.1}$ 
& \bfseries IBA$_{0.5}$ 
& \bfseries IBA$_1$ 
& \bfseries CoV \\
\hline
Cross-Entropy (CE)
& 0.7731 & 0.5899 & 0.5897
& 0.5558 & 0.4901 & 0.4097
& 0.3115 \\

Focal Loss \cite{lin2017focalloss}
& 0.7841 & 0.6098 & 0.5939
& 0.5378 & 0.4729 & 0.3916
& 0.3100 \\

LDAM Loss \cite{cao2019learning}
& 0.7798 & 0.6364 & 0.6392
& 0.5825 & 0.5168 & 0.4346
& 0.2460 \\

CB Loss \cite{cui2019balanced}
& 0.7615 & 0.6529 & 0.7270
& 0.6797 & 0.6182 & 0.5412
& 0.1060 \\

CCE Loss \cite{kim2021imbalanced}
& 0.7764 & 0.5861 & 0.5654
& 0.5090 & 0.4431 & 0.3607
& 0.3560 \\

PF Loss \cite{du2021parameter}
& 0.6479 & 0.5555 & 0.6968
& 0.6404 & 0.5774 & 0.4986
& 0.0890 \\

AWB Loss \cite{yue2022toward}
& 0.7174 & 0.6153 & 0.7111
& 0.6598 & 0.5960 & 0.5163
& 0.0750 \\

\end{tabular}
}
\end{table}


==> tables/combination_diffs.tex <==
\begin{table}[t]
\floatconts{tab:angular-only-results}
{\color{blue}\Caption{Angular Representation within Different Loss Functions}{
    We show the performance on the ISIC 2018 test set for several state-of-the-art loss functions with using the angular formulation in \eqref{eq:adacos} with $S=4$ and including our BAAM.
    Results are reported as the mean over five runs, and highest results per metric are highlighted in \textbf{bold}.
    In the second row of each metric, we show the absolute performance difference (in \% for better legibility, and major improvements marked in \textit{italics}) to the traditional dot-product-based logits as reported in \tabref{tab:test-isic-2018}.
    The results of our proposed DAL are copied from \tabref{tab:test-isic-2018} for easier reference.
}}
{
\scriptsize
\begin{tabular}{lrrrrrrr}
\bfseries Method 
& \multicolumn{1}{c}{\bfseries Acc}
& \multicolumn{1}{c}{\bfseries F1}
& \multicolumn{1}{c}{\bfseries BAcc }
& \multicolumn{1}{c}{\bfseries IBA$_{0.1}$ }
& \multicolumn{1}{c}{\bfseries IBA$_{0.5}$ }
& \multicolumn{1}{c}{\bfseries IBA$_1$ }
& \multicolumn{1}{c}{\bfseries CoV} \\
\hline

\multirow{2}{*}{Cross-Entropy (CE)}
 & 0.7731 & 0.5899 & 0.5897 & 0.5558 & 0.4901 & 0.4097 & 0.3115 \\
 & -0.5\% & -2.8\% & -1.2\% & +1.1\% & +1.4\% & +2.1\% & +0.0503 \\[1ex]

\multirow{2}{*}{Focal Loss \cite{lin2017focalloss}}
 & \bf 0.7841 & 0.6098 & 0.5939 & 0.5378 & 0.4729 & 0.3916 & 0.3100 \\
 & +1.2\% & -1.0\% & -1.6\% & -1.5\% & -1.1\% & -0.5\% & +0.0627 \\[1ex]

\multirow{2}{*}{LDAM Loss \cite{cao2019learning}}
 & 0.7798 & 0.6364 & 0.6392 & 0.5825 & 0.5168 & 0.4346 & 0.2460 \\
 & -0.7\% & -2.4\% & -2.9\% & -2.2\% & -2.1\% & -2.0\% & +0.0417 \\[1ex]

\multirow{2}{*}{CB Loss \cite{cui2019balanced}}
 & 0.7615 & \bf 0.6529 & 0.7270 & 0.6797 & 0.6182 & 0.5412 & 0.1060 \\
 & -1.5\% & -1.5\% & \it +5.4\% & \it +5.8\% & \it +6.6\% & \it +7.5\% & -0.0240 \\[1ex]

\multirow{2}{*}{CCE Loss \cite{kim2021imbalanced}}
 & 0.7764 & 0.5861 & 0.5654 & 0.5090 & 0.4431 & 0.3607 & 0.3560 \\
 & +0.3\% & -3.0\% & -4.3\% & -4.5\% & -4.2\% & -3.8\% & +0.1221 \\[1ex]

\multirow{2}{*}{PF Loss \cite{du2021parameter}}
 & 0.6479 & 0.5555 & 0.6968 & 0.6404 & 0.5774 & 0.4986 & 0.0890 \\
 & -8.8\% & -9.1\% & +0.3\% & -0.3\% & +0.1\% & +0.5\% & -0.0040 \\[1ex]

\multirow{2}{*}{AWB Loss \cite{yue2022toward}}
 & 0.7174 & 0.6153 & 0.7111 & 0.6598 & 0.5960 & 0.5163 & \bf 0.0750 \\
 & -1.4\% & -2.2\% & \it +6.1\% & \it +6.5\% & \it +7.1\% & \it +7.9\% & \it -0.0619 \\[.5ex]
\hline\\[-2ex]

DAL (Ours)
& 0.7443 & 0.6490 & \bf 0.7348 & \bf 0.6832 & \bf 0.6227 & \bf 0.5470 & 0.0972 \\
 
\end{tabular}
}
\end{table}


==> tables/distributions-s.tex <==
\begin{figure}[t]
\floatconts{fig:negative_angles_s_scales}
{\Caption{Negative Angles}{
    We show the distribution of negative angles $\theta_{i,j}$ during training on ISIC 2018 dataset with different $s$ parameter values, and including all training epochs.
}}
{
\subfigure[$s=3$]{\includegraphics[width=0.48\textwidth]{Figures/negative_angles_s3.pdf}}
\subfigure[$s=4$]{\includegraphics[width=0.48\textwidth]{Figures/negative_angles_s4.pdf}}

\subfigure[$s=8$]{\includegraphics[width=0.48\textwidth]{Figures/negative_angles_s8.pdf}}
\subfigure[$s=16$]{\includegraphics[width=0.48\textwidth]{Figures/negative_angles_s16.pdf}}\vspace*{-4ex}
}
\end{figure}


==> tables/hyperparameters.tex <==
\begin{table}[t]
\floatconts{tab:isic2018hyperparameters}
{\Caption{Ablation Study}{
    This table reports test-set performance for ArcFace models under different combinations of scale $s$, margin $m$, and dynamic weighted cross-entropy (DWCE).
    Metrics include overall accuracy (Acc), macro F1-score (F1), balanced accuracy (BAcc), and the imbalance-aware index (IBA) at three settings of $\alpha$, and the coefficient of variation (CoV). 
    The last column shows the p-values for a paired t-test comparing to our method.\vspace*{-4ex}
}}
{\scriptsize
\begin{tabular}{l@{\ \ }c@{\ \ }c@{\ \ }c|*{7}{c@{\ \ }}c}
\bfseries Method & \bfseries $s$ & \bfseries $m$ & \bfseries DWCE 
& \bfseries Acc & \bfseries F1 & \bfseries BAcc 
& \bfseries IBA$_{0.1}$ & \bfseries IBA$_{0.5}$ & \bfseries IBA$_1$
& \bfseries CoV & \bfseries p-value \\
\hline
ArcFace & 4 & 0.0 & No  & 0.7731 & 0.5899 & 0.5897 & 0.5558 & 0.4901 & 0.4097 & 0.3115 & \( \mathbf{4.464 \mathrm{e}{-6}} \) \\
ArcFace & 4 & 0.1 & No  & 0.7787 & 0.5847 & 0.5789 & 0.5398 & 0.4763 & 0.3894 & 0.3131 &\( \mathbf{1.576 \mathrm{e}{-6}} \) \\
ArcFace & 4 & 0.2 & No  & 0.7665 & 0.5781 & 0.5708 & 0.5144 & 0.4491 & 0.3675 & 0.3182 & \( \mathbf{2.387 \mathrm{e}{-7}} \) \\
ArcFace & 4 & 0.3 & No  & 0.7778 & 0.5835 & 0.5682 & 0.5121 & 0.4501 & 0.3726 & 0.3240 & \( \mathbf{1.741 \mathrm{e}{-7}} \) \\
ArcFace & 8   & 0.0 & No  & 0.7837 & 0.6385 & 0.6148 & 0.5591 & 0.4887 & 0.4007 & 0.3022 & \( \mathbf{3.482 \mathrm{e}{-7}} \) \\
ArcFace & 8   & 0.1 & No  & 0.7804 & 0.6384 & 0.6134 & 0.5571 & 0.4859 & 0.3969 & 0.3019 & \( \mathbf{3.123 \mathrm{e}{-7}} \) \\
ArcFace & 8   & 0.2 & No  & \textbf{0.7943} & 0.6663 & 0.6380 & 0.5821 & 0.5123 & 0.4251 & 0.2771 & \( \mathbf{2.193 \mathrm{e}{-6}} \) \\
ArcFace & 8   & 0.3 & No  & 0.7798 & 0.6305 & 0.6036 & 0.5477 & 0.4779 & 0.3907 & 0.2947 & \( \mathbf{1.385 \mathrm{e}{-6}} \) \\
ArcFace & 16  & 0.1 & No  & 0.7712 & 0.6116 & 0.6103 & 0.5556 & 0.4854 & 0.3976 & 0.2599 & \( \mathbf{1.441 \mathrm{e}{-6}} \) \\
ArcFace & 16  & 0.2 & No  & 0.7851 & 0.6375 & 0.6101 & 0.5504 & 0.4810 & 0.3943 & 0.2546 & \( \mathbf{1.491 \mathrm{e}{-6}} \) \\
ArcFace & 16  & 0.3 & No  & 0.7824 & 0.6536 & 0.6571 & 0.6034 & 0.5350 & 0.4495 & 0.2114 & \( \mathbf{1.195 \mathrm{e}{-5}} \) \\
\hline
CE & -  & - & \textcolor{blue}{Yes}  & \textcolor{blue}{0.7630} & \textcolor{blue}{0.6606} & \textcolor{blue}{0.6820} & \textcolor{blue}{0.6323} & \textcolor{blue}{0.5645} & \textcolor{blue}{0.4798} & \textcolor{blue}{0.134} & \( \textcolor{blue}{\mathbf{1.005 \mathrm{e}{-4}} }\) \\
\hline
ArcFace & 4   & 0.0 & Yes & 0.7553 & 0.6458 & 0.7248 & 0.6767 & 0.6152 & 0.5432 & 0.1068 & \( \mathbf{4.214 \mathrm{e}{-3}} \) \\
ArcFace & 4   & 0.1 & Yes & 0.7665 & 0.6580 & 0.7103 & 0.6594 & 0.5910 & 0.5101 & 0.1138 & \( \mathbf{1.615 \mathrm{e}{-3}} \) \\
ArcFace & 4   & 0.2 & Yes & 0.7595 & 0.6601 & 0.7060 & 0.6494 & 0.5830 & 0.5032 & 0.1223 & \( \mathbf{1.211 \mathrm{e}{-3}} \) \\
ArcFace & 4   & 0.3 & Yes & 0.7684 & 0.6618 & 0.6989 & 0.6411 & 0.5749 & 0.4992 & 0.1049 & \( \mathbf{5.213 \mathrm{e}{-4}} \) \\
ArcFace & 8   & 0.0 & Yes & 0.7524 & 0.6512 & 0.7139 & 0.6619 & 0.5999 & 0.5131 & 0.1198 & \( \mathbf{2.231 \mathrm{e}{-3}} \) \\
ArcFace & 8   & 0.1 & Yes & 0.7559 & 0.6604 & 0.7197 & 0.6698 & 0.6085 & 0.5271 & \textbf{0.0876} & \( \mathbf{3.112 \mathrm{e}{-3}} \) \\
ArcFace & 8   & 0.2 & Yes & 0.7617 & 0.6659 & 0.7143 & 0.6641 & 0.6009 & 0.5203 & 0.0932 & \( \mathbf{2.788 \mathrm{e}{-3}} \) \\
ArcFace & 8   & 0.3 & Yes & 0.7467 & 0.6388 & 0.7010 & 0.6449 & 0.5838 & 0.5010 & 0.0959 & \( \mathbf{1.528 \mathrm{e}{-3}} \) \\
ArcFace & 16  & 0.0 & Yes & 0.7521 & 0.6634 & 0.6910 & 0.6377 & 0.5718 & 0.4894 & 0.0998 & \( \mathbf{6.342 \mathrm{e}{-4}} \) \\
ArcFace & 16  & 0.1 & Yes & 0.7591 & 0.6511 & 0.6890 & 0.6356 & 0.5701 & 0.4927 & 0.1059 & \( \mathbf{1.687 \mathrm{e}{-4}} \) \\
ArcFace & 16  & 0.2 & Yes & 0.7648 & 0.6659 & 0.6979 & 0.6496 & 0.5813 & 0.4988 & 0.1022 & \( \mathbf{5.124 \mathrm{e}{-4}} \) \\
ArcFace & 16  & 0.3 & Yes & 0.7698 & \textbf{0.6761} & 0.7095 & 0.6576 & 0.5889 & 0.5090 & 0.0938 & \( \mathbf{1.442 \mathrm{e}{-3}} \) \\
\hline
\textcolor{blue}{AdaCos} (fixed) & \textcolor{blue}{2.56} & \textcolor{blue}{0.0} & \textcolor{blue}{Yes} & \textcolor{blue}{0.7251} & \textcolor{blue}{0.6162} & \textcolor{blue}{0.7204} & \textcolor{blue}{0.6714} & \textcolor{blue}{0.6093} & \textcolor{blue}{0.5316} & \textcolor{blue}{0.1050} & \(\textcolor{blue}{\mathbf{3.418 \mathrm{e}{-3}}} \) \\
AdaCos & dyn & 0.0 & Yes & 0.7163 & 0.6044 & 0.7018 & 0.6502 & 0.5850 & 0.5034 & 0.1348 & \( \mathbf{1.712 \mathrm{e}{-3}} \) \\
\hline
\textbf{DAL (Ours)} 
& 4 & var & Yes 
& 0.7443 & 0.6490 & \textbf{0.7348} 
& \textbf{0.6832} & \textbf{0.6227} & \textbf{0.5470} & 0.0930 
& \textbf{-} \\
\end{tabular}
}
\end{table}

==> tables/perclass_validation.tex <==
\begin{table}[t]
\floatconts{tab:perclass-validation}
{\Caption {Per-Class Recall}{ 
    This table shows the per-class recall aka.~True Positive Rate (TPR) on the validation set.
    Bold numbers highlight best values.\vspace*{-4ex}
}}

{
\subtable[ISIC 2018\label{tab:perclass-isic-validation-2018}]{
  \scriptsize
  \begin{tabular}{lccccccc}
  \bfseries Method 
  & \bfseries NV 
  & \bfseries MEL 
  & \bfseries BKL 
  & \bfseries BCC 
  & \bfseries AK
  & \bfseries VASC 
  & \bfseries DF \\
  \hline
%
  Cross-Entropy (CE)
  & 0.9327 & 0.5925 & 0.7054 & 0.6580 & 0.6157 & 0.7414 & 0.3478 \\
%
  Focal Loss \cite{lin2017focalloss}
  & \textbf{0.9369} & 0.5650 & 0.6786 & 0.7264 & 0.5970 & 0.7672 & 0.3487 \\
%
  LDAM Loss \cite{cao2019learning}
  & 0.9289 & 0.6134 & 0.6930 & 0.7759 & 0.5895 & 0.9123 & 0.6741 \\
%
  CB Loss \cite{cui2019balanced}
  & 0.8920 & \textbf{0.6740} & 0.7046 & 0.7436 & 0.5617 & 0.9142 & 0.6712 \\
%
  CCE Loss \cite{kim2021imbalanced}
  & 0.9359 & 0.5733 & 0.6679 & 0.7099 & 0.6113 & 0.7784 & 0.3804 \\
%
  PF Loss \cite{du2021parameter}
  & 0.7910 & 0.6718 & \textbf{0.7369} & 0.7899 & 0.7227 & 0.9379 & 0.7048 \\
%
  AWB Loss \cite{yue2022toward}
  & 0.8689 & 0.6711 & 0.7321 & \textbf{0.7956} & 0.6468 & 0.9540 & 0.6722 \\
%
  DAL (Ours)
  & 0.8086 & 0.6582 & 0.6948 & 0.7834 & \textbf{0.7612} & \textbf{0.9766} & \textbf{0.7578} \\
%
  \end{tabular}}

\subtable[ISIC 2019\label{tab:perclass-isic-validation-2019}]{\scriptsize
  \begin{tabular}{lcccccccc}
  \bfseries Method 
  & \bfseries NV 
  & \bfseries MEL 
  & \bfseries BCC 
  & \bfseries BKL 
  & \bfseries AK 
  & \bfseries SCC 
  & \bfseries VASC 
  & \bfseries DF \\
  \hline
  Cross-Entropy (CE)
  & \textbf{0.8973} & 0.6604 & 0.7521 & 0.5962 & 0.4942 & 0.4061 & 0.6536 & 0.3403 \\
%
  Focal Loss \cite{lin2017focalloss}
  & 0.8948 & 0.6377 & 0.7758 & 0.5843 & 0.5395 & 0.4289 & 0.6118 & 0.3504 \\
%
  LDAM Loss \cite{cao2019learning}
  & 0.8821 & 0.6842 & 0.8263 & 0.5910 & 0.4118 & 0.4623 & 0.8284 & 0.5990 \\
%
  CB Loss \cite{cui2019balanced}
  & 0.8366 & 0.6327 & 0.7822 & 0.6133 & 0.5708 & 0.5992 & 0.8284 & 0.6922 \\
%
  CCE Loss \cite{kim2021imbalanced}
  & 0.8927 & 0.6388 & 0.7763 & 0.6015 & 0.4704 &  0.3723 & 0.7353 & 0.3221 \\
%
  PF Loss \cite{du2021parameter}
  & 0.7866 & 0.6517 & 0.7980 & 0.6147 & 0.5984 & 0.5794 & 0.8984 & 0.7125 \\
%
  AWB Loss \cite{yue2022toward}
  & 0.7804 & \textbf{0.6881} & \textbf{0.8440} & 0.6338 & 0.5650 & 0.5992 & \textbf{0.9216} & 0.6615 \\
%
  DAL (Ours)
  & 0.7270 & 0.6426 & 0.7365 & \textbf{0.6367} & \textbf{0.6317} & \textbf{0.6308} & 0.9176 & \textbf{0.7375} \\
%
  \end{tabular}}

% \subtable[APTOS \label{tab:perclass-validation-aptos}]{\scriptsize
%   \begin{tabular}{lccccc}
%   \bfseries Method 
%   & \bfseries No DR
%   & \bfseries Moderate
%   & \bfseries Mild
%   & \bfseries Proliferative DR
%   & \bfseries Severe \\
%   \hline
% %
%   Cross-Entropy (CE)
%   &  &  &  &  &  \\
% %
%   Focal Loss \cite{lin2017focalloss}
%   &  &  &  &  &  \\
% %
%   LDAM Loss \cite{cao2019learning}
%   &  &  &  &  &  \\
% %
%   CB Loss \cite{cui2019balanced}
%   &  &  &  &  &  \\
% %
%   CCE Loss \cite{kim2021imbalanced}
%   &  &  &  &  &  \\
% %
%   PF Loss \cite{du2021parameter}
%   &  &  &  &  &  \\
% %
%   AWB Loss \cite{yue2022toward}
%   &  &  &  &  &  \\
% %
%   Ours
%    &  &  &  &  &  \\
% %
%   \end{tabular}}
}
\end{table}


==> tables/performace_validation.tex <==
\begin{table}[t]
\floatconts{tab:validation-results}
{\Caption{Validation Set Performance}{
    This table shows results obtained on the validation sets, providing the mean over 5 runs on two datasets.
    Best results are highlighted in bold.\vspace*{-4ex}
}}
{
\subtable[ISIC 2018\label{tab:validation-isic-2018}]{\scriptsize
  \begin{tabular}{lccccccc}
  \bfseries Method 
  & \bfseries Acc 
  & \bfseries F1 
  & \bfseries BAcc 
  & \bfseries IBA$_{0.1}$ 
  & \bfseries IBA$_{0.5}$ 
  & \bfseries IBA$_1$ 
  & \bfseries CV\\
  \hline
  Cross-Entropy (CE)
  & 0.8356 & 0.6662 & 0.6531 
  & 0.6030 & 0.5376 & 0.4559 
  & 0.2490 \\
%
  Focal Loss \cite{lin2017focalloss}
  & 0.8341 & 0.6739 & 0.6597 
  & 0.6091 & 0.5454 & 0.4657 
  & 0.2594 \\
%
  LDAM Loss \cite{cao2019learning}
  & \textbf{0.8598} & 0.7211 & 0.7429 
  & 0.6976 & 0.6433 & 0.5754 
  & 0.2008 \\
%
  CB Loss \cite{cui2019balanced}
  & 0.8267 & \textbf{0.7243} & 0.7351 
  & 0.6838 & 0.6254 & 0.5593 
  & 0.1664 \\
%
  CCE Loss \cite{kim2021imbalanced}
  & 0.8358 & 0.6871 & 0.6770 
  & 0.6140 & 0.5503 & 0.4705 
  & 0.2531 \\
%
  PF Loss \cite{du2021parameter}
  & 0.7798 & 0.6985 & 0.7649 
  & 0.7139 & 0.6618 & 0.5958 
  & 0.1170 \\
%
  AWB Loss \cite{yue2022toward}
  & 0.7929 & 0.7169 & 0.7591 
  & 0.7118 & 0.6589 & 0.5928 
  & 0.1513 \\
 %  
  DAL (Ours)
  & 0.7743 & 0.6787 & \textbf{0.7771} 
  & \textbf{0.7321} & \textbf{0.6832} & \textbf{0.6132}   & \textbf{0.1434} \\
%
  \end{tabular}}

\subtable[ISIC 2019\label{tab:validation-isic-2019}]{\scriptsize
  \begin{tabular}{lccccccc}
  \bfseries Method 
  & \bfseries Acc 
  & \bfseries F1 
  & \bfseries BAcc 
  & \bfseries IBA$_{0.1}$ 
  & \bfseries IBA$_{0.5}$ 
  & \bfseries IBA$_1$ 
  & \bfseries CV\\
  \hline
  Cross-Entropy (CE)
  & 0.7703 & 0.6023 & 0.6013 
  & 0.5539 & 0.4830 & 0.3945 
  & 0.2903\\
%
  Focal Loss \cite{lin2017focalloss}
  & 0.7686 & 0.6067 & 0.6037 
  & 0.5566 & 0.4838 & 0.3954 
  & 0.2816\\
%
  LDAM Loss \cite{cao2019learning}
  & \textbf{0.7796} & 0.6557 & 0.6606 
  & 0.6149 & 0.5501 & 0.4691 
  & 0.2557\\
%
  CB Loss \cite{cui2019balanced}
  & 0.7536 & 0.6670 & 0.6941 
  & 0.6482 & 0.5823 & 0.4994 
  & 0.1504\\
%  
  CCE Loss \cite{kim2021imbalanced}
  & 0.7671 & 0.6043 & 0.5998 
  & 0.5524 & 0.4851 & 0.4010 
  & 0.2977\\
%
  PF Loss \cite{du2021parameter}
  & 0.7357 & 0.6540 & 0.7043 
  & 0.6584 & 0.5950 & 0.5153 
  & 0.1607\\
%
  AWB Loss \cite{yue2022toward}
  & 0.7476 & \textbf{0.6864} & \textbf{0.7117} 
  & \textbf{0.6649} & \textbf{0.6035} & \textbf{0.5267} 
  & 0.1644\\
%
  DAL (Ours)
  & 0.7149 & 0.6024 & 0.7068 
  & 0.6552 & 0.5959 & 0.5167 
  & \textbf{0.1255}\\
%
  \end{tabular}}

% \subtable[APTOS\label{tab:validation-aptos}]{\scriptsize
%   \begin{tabular}{lccccccc}
%   \bfseries Method 
%   & \bfseries Acc 
%   & \bfseries F1 
%   & \bfseries BAcc 
%   & \bfseries IBA$_{0.1}$ 
%   & \bfseries IBA$_{0.5}$ 
%   & \bfseries IBA$_1$ 
%   & \bfseries CV \\
%   \hline
%   Cross-Entropy (CE)
%   &  &  &  
%   &  &  &  
%   & \\
% %
%   Focal Loss \cite{lin2017focalloss}
%   &  &  &  
%   &  &  &  
%   & \\
% %
%   LDAM Loss \cite{cao2019learning}
%   &  &  &  
%   &  &  &  
%   & \\
% %
%   CB Loss \cite{cui2019balanced}
%   &  &  &  
%   &  &  &  
%   & \\
% %
%   CCE LOss \cite{kim2021imbalanced}
%   &  &  &  
%   &  &  &  
%   & \\
% %
%   PF Loss \cite{du2021parameter}
%   &  &  &  
%   &  &  &  
%   & \\
% %
%   AWB Loss \cite{yue2022toward}
%   &  &  &  
%   &  &  &  
%   & \\
% %
%   Ours
%   &  &  &  
%   &  &  &  
%   & \\
% %
%   \end{tabular}}
}
\end{table}


==> tables/performance.tex <==
\begin{table}[t]\centering
\Caption[tab:test-results]{Test Set Performance}{
    We show test set results across all methods, providing the mean over 5 runs on three datasets.
    Best results are highlighted in bold.
}
\iffalse
\subfloat[ISIC 2018]{\label{tab:test-isic-2018}\scriptsize
  \begin{tabular}{lccccccc}
  \bfseries Method 
  & \bfseries Acc 
  & \bfseries F1 
  & \bfseries BAcc 
  & \bfseries IBA$_{0.1}$ 
  & \bfseries IBA$_{0.5}$ 
  & \bfseries IBA$_1$ 
  & \bfseries CoV\\
  \hline
  Cross-Entropy (CE)
  & 0.7779 & 0.6182 & 0.6015 
  & 0.5451 & 0.4756 & 0.3887 
  & 0.2612 \\
%
  Focal Loss \cite{lin2017focalloss}
  & 0.7722 & 0.6195 & 0.6095 
  & 0.5531 & 0.4837 & 0.3969 
  & 0.2473 \\
%
  LDAM Loss \cite{cao2019learning}
  & \textbf{0.7864} & 0.6603 & 0.6678 
  & 0.6045 & 0.5379 & 0.4547 
  & 0.2043 \\
%
  CB Loss \cite{cui2019balanced}
  & 0.7763 & \textbf{0.6680} & 0.6730 
  & 0.6216 & 0.5524 & 0.4659 
  & 0.1300 \\
%
  CCE Loss \cite{kim2021imbalanced}
  & 0.7738 & 0.6162 & 0.6084 
  & 0.5536 & 0.4850 & 0.3991 
  & 0.2339 \\
%
  PF Loss \cite{du2021parameter}
  & 0.7357 & 0.6465 & 0.6941 
  & 0.6435 & 0.5769 & 0.4936 
  & \textbf{0.0930} \\
%
  AWB Loss \cite{yue2022toward}
  & 0.7312 & 0.6368 & 0.6500 
  & 0.5950 & 0.5250 & 0.4375 
  & 0.1369 \\
 %  
  DAL (Ours)
  & 0.7443 & 0.6490 & \textbf{0.7348} 
  & \textbf{0.6832} & \textbf{0.6227} & \textbf{0.5470} 
  & 0.0972 \\
%
  \end{tabular}}
\fi

\subfloat[ISIC 2019\label{tab:test-isic-2019}]{\scriptsize
  \begin{tabular}{lccccccc}
  \bfseries Method 
  & \bfseries Acc$\uparrow$ 
  & \bfseries F1$\uparrow$  
  & \bfseries BAcc$\uparrow$  
  & \bfseries IBA$_{0.1}$$\uparrow$  
  & \bfseries IBA$_{0.5}$$\uparrow$  
  & \bfseries IBA$_1$$\uparrow$  
  & \bfseries CoV$\downarrow$ \\
  \hline
  Cross-Entropy (CE)
  & 0.6378 & 0.4633 & 0.4562 
  & 0.4044 & 0.3381 & 0.2551 
  & 0.4329 \\
%
  Focal Loss \cite{lin2017focalloss}
  & 0.6466 & 0.4792 & 0.4687 
  & 0.4139 & 0.3470 & 0.2634 
  & 0.4226 \\
%
  AdaCos \cite{zhang2019adacos}
  & 0.6379 & 0.3661 & 0.3817
  & 0.3077 & 0.2715 & 0.2263
  & 0.7855 \\
%
  ArcFace \cite{deng2022arcface}
  & 0.6434 & 0.4517 & 0.4239
  & 0.3711 & 0.3139 & 0.2424
  & 0.6003 \\
%
  LDAM Loss \cite{cao2019learning}
  & 0.6319 & 0.4759 & 0.4798 
  & 0.4267 & 0.3642 & 0.2869 
  & 0.3298 \\
%
  DWCE Loss & 0.6392 & 0.5089 & 0.5029 
  & 0.4512 & 0.3792 & 0.2891 
  & 0.3501 \\
%
  CB Loss \cite{cui2019balanced}
  & \textbf{0.6472} & 0.5105 & 0.4970 
  & 0.4448 & 0.3752 & 0.2881 
  & 0.3632 \\
%  
  CCE Loss \cite{kim2021imbalanced}
  & 0.6467 & 0.4756 & 0.4576 
  & 0.4053 & 0.3395 & 0.2574 
  & 0.4415 \\
%
  PF Loss \cite{du2021parameter}
  & 0.6308 & 0.5029 & 0.5233 
  & 0.4721 & 0.3974 & 0.3040 
  & 0.2701 \\
%
  AWB Loss \cite{yue2022toward}
  & 0.6292 & \textbf{0.5134} & 0.5045 
  & 0.4500 & 0.3805 & 0.2937 
  & 0.3508 \\
%
  DCAL \cite{kim2025long}
  & 0.6328 & 0.4886 & 0.4812
  & 0.4282 & 0.3584 & 0.2711
  & 0.3908 \\
%
  DAL (Ours)
  & 0.6114 & 0.5003 & \textbf{0.5545} 
  & \textbf{0.4993} & \textbf{0.4264} & \textbf{0.3343} 
  & \textbf{0.1872} \\
%
  \end{tabular}}

\subfloat[APTOS\label{tab:test-aptos}]{\scriptsize
  \begin{tabular}{lccccccc}
  \bfseries Method 
  & \bfseries Acc$\uparrow$ 
  & \bfseries F1$\uparrow$  
  & \bfseries BAcc$\uparrow$  
  & \bfseries IBA$_{0.1}$$\uparrow$  
  & \bfseries IBA$_{0.5}$$\uparrow$  
  & \bfseries IBA$_1$$\uparrow$  
  & \bfseries CoV$\downarrow$ \\
  \hline
  Cross-Entropy (CE)
  & 0.8175 & 0.6163 & 0.6047 
  & 0.5568 & 0.5139 & 0.4602 
  & 0.4990 \\
%
  Focal Loss \cite{lin2017focalloss}
  & \textbf{0.8292} & 0.6286 & 0.6111 
  & 0.5655 & 0.5214 & 0.4664 
  & 0.4899 \\
%
   AdaCos \cite{zhang2019adacos}
   & 0.7722 & 0.3661 & 0.3817
   & 0.3077 & 0.2715 & 0.2263
   & 0.7855 \\
%
  ArcFace \cite{deng2022arcface}
  & 0.6434 & 0.4517 & 0.4239
  & 0.3711 & 0.3139 & 0.2424
  & 0.6003 \\
%
  LDAM Loss \cite{cao2019learning}
  & 0.8002 & 0.6321 & 0.6287 
  & 0.5821 & 0.5293 & 0.4697 
  & 0.3986 \\
%
  DWCE Loss 
  & 0.7965 & 0.6238 & 0.6354 
  & 0.5796 & 0.5208 & 0.4523 
  & 0.3225 \\
%
  CB Loss \cite{cui2019balanced}
  & 0.8028 & 0.6319 & 0.6439 
  & 0.5889 & 0.5312 & 0.4621 
  & 0.3092 \\
%
  CCE LOss \cite{kim2021imbalanced}
  & 0.7999 & 0.5794 & 0.5748 
  & 0.5284 & 0.4851 & 0.4309 
  & 0.5331 \\
%
  PF Loss \cite{du2021parameter}
  & 0.7902 & 0.6349 & 0.6410 
  & 0.5902 & 0.5347 & 0.4653 
  & 0.3189 \\
%
  AWB Loss \cite{yue2022toward}
  & 0.8016 & \textbf{0.6491} & 0.6481 
  & 0.5993 & 0.5407 & 0.4674 
  & 0.3047 \\
%
  DCAL \cite{kim2025long}
  & 0.8018 & 0.6224 & 0.6118
  & 0.5630 & 0.5085 & 0.4405
  & 0.4471 \\
%
  DAL (Ours)
  & 0.7793 & 0.6337 & \textbf{0.6756} 
  & \textbf{0.6248} & \textbf{0.5659} & \textbf{0.4923} 
  & \textbf{0.2397} \\
%
  \end{tabular}}  

\end{table}

